Domain walls and M2-branes partition functions: M-theory and ABJM Theory

We study the BPS counting functions (free energies) of the M-string configurations. We consider separated M5-branes along with M2-branes stretched between them, with M5-branes acting as domain walls interpolating different configurations of M2-branes. We find recursive structure in the free energies of these configurations. The M-string degrees of freedom on the domain walls are interpreted in terms of a pair of interacting supersymmetric WZW models. We also compute the elliptic genus of the M-string in a toy model of the ABJM theory and compare it with the M-theory computation.

==> bibliography.tex <==
@article{Witten:1993jg,
    author = "Witten, Edward",
    title = "{On the Landau-Ginzburg description of N=2 minimal models}",
    eprint = "hep-th/9304026",
    archivePrefix = "arXiv",
    reportNumber = "IASSNS-HEP-93-10",
    doi = "10.1142/S0217751X9400193X",
    journal = "Int. J. Mod. Phys. A",
    volume = "9",
    pages = "4783--4800",
    year = "1994"
}
@article{Katz:2002gh,
    author = "Katz, Sheldon H. and Sharpe, Eric",
    title = "{D-branes, open string vertex operators, and Ext groups}",
    eprint = "hep-th/0208104",
    archivePrefix = "arXiv",
    reportNumber = "ILL-TH-02-06, ILL-(TH)-02-06",
    doi = "10.4310/ATMP.2002.v6.n6.a1",
    journal = "Adv. Theor. Math. Phys.",
    volume = "6",
    pages = "979--1030",
    year = "2003"
}
@article{Nemeschansky:1994ac,
    author = "Nemeschansky, D. and Warner, N. P.",
    title = "{The Refined elliptic genus and Coulomb gas formulations of N=2 superconformal coset models}",
    eprint = "hep-th/9412187",
    archivePrefix = "arXiv",
    reportNumber = "USC-94-018, CERN-TH-7548-94",
    doi = "10.1016/0550-3213(95)00059-2",
    journal = "Nucl. Phys. B",
    volume = "442",
    pages = "623--654",
    year = "1995"
}
@article{Berglund:1993fj,
    author = "Berglund, Per and Henningson, Mans",
    title = "{Landau-Ginzburg orbifolds, mirror symmetry and the elliptic genus}",
    eprint = "hep-th/9401029",
    archivePrefix = "arXiv",
    reportNumber = "IASSNS-HEP-93-92",
    doi = "10.1016/0550-3213(94)00389-V",
    journal = "Nucl. Phys. B",
    volume = "433",
    pages = "311--332",
    year = "1995"
}
@article{Henningson:1993nr,
    author = "Henningson, Mans",
    title = "{N=2 gauged WZW models and the elliptic genus}",
    eprint = "hep-th/9307040",
    archivePrefix = "arXiv",
    reportNumber = "IASSNS-HEP-93-39",
    doi = "10.1016/0550-3213(94)90614-9",
    journal = "Nucl. Phys. B",
    volume = "413",
    pages = "73--83",
    year = "1994"
}

@article{Aganagic:2003db,
    author = "Aganagic, Mina and Klemm, Albrecht and Marino, Marcos and Vafa, Cumrun",
    title = "{The Topological vertex}",
    eprint = "hep-th/0305132",
    archivePrefix = "arXiv",
    reportNumber = "CALT-68-2439, HUTP-03-A032, HU-EP-03-24, CERN-TH-2003-111",
    doi = "10.1007/s00220-004-1162-z",
    journal = "Commun. Math. Phys.",
    volume = "254",
    pages = "425--478",
    year = "2005"
}
@article{Benini:2018hjy,
    author = "Benini, Francesco and Bonelli, Giulio and Poggi, Matteo and Tanzini, Alessandro",
    title = "{Elliptic non-Abelian Donaldson-Thomas invariants of $\mathbb{C}^3$}",
    eprint = "1807.08482",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SISSA 29/2018/FISI",
  %  doi = "10.1007/JHEP07(2019)068",
%    journal = "JHEP",
%    volume = "07",
%    pages = "068",
%    year = "2019"
}
@article{Gaiotto:2008ak,
    author = "Davide Gaiotto and Edward Witten ",
    title = "{S-Duality of Boundary Conditions In N=4 Super Yang-Mills Theory}",
    eprint = "0807.3720",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.4310/ATMP.2009.v13.n3.a5",
    journal = "Adv. Theor. Math. Phys.",
    volume = "13",
    number = "3",
    pages = "721--896",
    year = "2009"
}
@article{Hohenegger:2016eqy,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Self-Duality and Self-Similarity of Little String Orbifolds}",
    eprint = "1605.02591",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.94.046006",
    journal = "Phys. Rev. D",
    volume = "94",
    number = "4",
    pages = "046006",
    year = "2016"
}
@article{DelZotto:2014hpa,
    author = "Del Zotto, Michele and Heckman, Jonathan J. and Tomasiello, Alessandro and Vafa, Cumrun",
    title = "{6d Conformal Matter}",
    eprint = "1407.6359",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP02(2015)054",
    journal = "JHEP",
    volume = "02",
    pages = "054",
    year = "2015"
}
@article{Morrison:2012np,
    author = "Morrison, David R. and Taylor, Washington",
    title = "{Classifying bases for 6D F-theory models}",
    eprint = "1201.1943",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "UCSB-MATH-2012-01, MIT-CTP-4339",
    doi = "10.2478/s11534-012-0065-4",
    journal = "Central Eur. J. Phys.",
    volume = "10",
    pages = "1072--1088",
    year = "2012"
}
@article{Noumab,
    author = "Nouman Muteeb",
    title = "{in preparation}",
}
@article{Hosomichi:2014rqa,
    author = "Hosomichi, Kazuo and Lee, Sungjay",
    title = "{Self-dual Strings and 2D SYM}",
    eprint = "1406.1802",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "EFI-14-11, YITP-14-43",
    doi = "10.1007/JHEP01(2015)076",
    journal = "JHEP",
    volume = "01",
    pages = "076",
    year = "2015"
}
@article{Benini:2013xpa,
    author = "Benini, Francesco and Eager, Richard and Hori, Kentaro and Tachikawa, Yuji",
    title = "{Elliptic Genera of 2d ${\mathcal{N}}$ = 2 Gauge Theories}",
    eprint = "1308.4896",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "IPMU-13-0146, UT-13-29",
    doi = "10.1007/s00220-014-2210-y",
    journal = "Commun. Math. Phys.",
    volume = "333",
    number = "3",
    pages = "1241--1286",
    year = "2015"
}
@article{Benini:2013nda,
    author = "Benini, Francesco and Eager, Richard and Hori, Kentaro and Tachikawa, Yuji",
    title = "{Elliptic genera of two-dimensional N=2 gauge theories with rank-one gauge groups}",
    eprint = "1305.0533",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "IPMU-13-0082, UT-13-17",
    doi = "10.1007/s11005-013-0673-y",
    journal = "Lett. Math. Phys.",
    volume = "104",
    pages = "465--493",
    year = "2014"
}
@article{Gopakumar:1998ii,
    author = "Gopakumar, Rajesh and Vafa, Cumrun",
    title = "{M theory and topological strings. 1.}",
    eprint = "hep-th/9809187",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-98-A069",
    month = "9",
    year = "1998"
}
@article{Gopakumar:1998jq,
    author = "Gopakumar, Rajesh and Vafa, Cumrun",
    title = "{M theory and topological strings. 2.}",
    eprint = "hep-th/9812127",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-98-A070",
    month = "12",
    year = "1998"
}
@article{Gadde:2013dda,
    author = "Gadde, Abhijit and Gukov, Sergei",
    title = "{2d Index and Surface operators}",
    eprint = "1305.0266",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CALT-68.2932",
    doi = "10.1007/JHEP03(2014)080",
    journal = "JHEP",
    volume = "03",
    pages = "080",
    year = "2014"
}
@article{Gadde:2015tra,
    author = "Gadde, Abhijit and Haghighat, Babak and Kim, Joonho and Kim, Seok and Lockhart, Guglielmo and Vafa, Cumrun",
    title = "{6d String Chains}",
    eprint = "1504.04614",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP02(2018)143",
    journal = "JHEP",
    volume = "02",
    pages = "143",
    year = "2018"
}
@article{Nakajima:2003pg,
    author = "Nakajima, Hiraku and Yoshioka, Kota",
    title = "{Instanton counting on blowup. 1.}",
    eprint = "math/0306198",
    archivePrefix = "arXiv",
    doi = "10.1007/s00222-005-0444-1",
    journal = "Invent. Math.",
    volume = "162",
    pages = "313--355",
    year = "2005"
}
@article{Bastian:2019hpx,
    author = "Bastian, Brice and Hohenegger, Stefan",
    title = "{Symmetries in A-type little string theories. Part I. Reduced free energy and paramodular groups}",
    eprint = "1911.07276",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP03(2020)062",
    journal = "JHEP",
    volume = "03",
    pages = "062",
    year = "2020"
}
@article{Bastian:2019wpx,
    author = "Bastian, Brice and Hohenegger, Stefan",
    title = "{Symmetries in A-type little string theories. Part II. Eisenstein series and generating functions of multiple divisor sums}",
    eprint = "1911.07280",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP03(2020)016",
    journal = "JHEP",
    volume = "03",
    pages = "016",
    year = "2020"
}
@misc{zwegers2008mock,
      title={Mock Theta Functions}, 
      author={Sander Zwegers},
      year={2008},
      eprint={0807.4834},
      archivePrefix={arXiv},
      primaryClass={math.NT}
}
@inproceedings{Sharpe:2003dr,
    author = "Sharpe, Eric",
    title = "{Lectures on D-branes and sheaves}",
    eprint = "hep-th/0307245",
    archivePrefix = "arXiv",
    reportNumber = "ILL-TH-03-6",
    month = "7",
    year = "2003"
}
@article{Gopakumar:1998jq,
    author = "Gopakumar, Rajesh and Vafa, Cumrun",
    title = "{M theory and topological strings. 2.}",
    eprint = "hep-th/9812127",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-98-A070",
    month = "12",
    year = "1998"
}
@article{Gopakumar:1998ii,
    author = "Gopakumar, Rajesh and Vafa, Cumrun",
    title = "{M theory and topological strings. 1.}",
    eprint = "hep-th/9809187",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-98-A069",
    month = "9",
    year = "1998"
}
@article{Haghighat:2013tka,
    author = "Haghighat, Babak and Kozcaz, Can and Lockhart, Guglielmo and Vafa, Cumrun",
    title = "{Orbifolds of M-strings}",
    eprint = "1310.1185",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.89.046003",
    journal = "Phys. Rev. D",
    volume = "89",
    number = "4",
    pages = "046003",
    year = "2014"
}
@article{Haghighat:2015coa,
    author = "Haghighat, Babak",
    title = "{From strings in 6d to strings in 5d}",
    eprint = "1502.06645",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP01(2016)062",
    journal = "JHEP",
    volume = "01",
    pages = "062",
    year = "2016"
}
@inproceedings{Nekrasov:2009rc,
    author = "Nekrasov, Nikita A. and Shatashvili, Samson L.",
    title = "{Quantization of Integrable Systems and Four Dimensional Gauge Theories}",
    booktitle = "{16th International Congress on Mathematical Physics}",
    eprint = "0908.4052",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "TCD-MATH-09-19, HMI-09-09, IHES-P-09-38",
    doi = "10.1142/9789814304634_0015",
    pages = "265--289",
    month = "8",
    year = "2009"
}
@article{Hohenegger:2015cba,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{M-strings, monopole strings, and modular forms}",
    eprint = "1503.06983",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SNUST-15-02",
    doi = "10.1103/PhysRevD.92.066005",
    journal = "Phys. Rev. D",
    volume = "92",
    number = "6",
    pages = "066005",
    year = "2015"
}
@article{Hohenegger:2015btj,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Instanton-monopole correspondence from M-branes on $\mathbb S^1$ and little string theory}",
    eprint = "1511.02787",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.93.066016",
    journal = "Phys. Rev. D",
    volume = "93",
    number = "6",
    pages = "066016",
    year = "2016"
}
@article{Okazaki:2015fiq,
    author = "Okazaki, Tadashi and Smith, Douglas J.",
    title = "{Topological M-strings and supergroup Wess-Zumino-Witten models}",
    eprint = "1512.06646",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DCPT-15-69, NCTS-TH-1508",
    doi = "10.1103/PhysRevD.94.065016",
    journal = "Phys. Rev. D",
    volume = "94",
    number = "6",
    pages = "065016",
    year = "2016"
}
@article{Okazaki:2016pne,
    author = "Okazaki, Tadashi and Smith, Douglas J.",
    title = "{Mock modular index of M2-M5 brane systems}",
    eprint = "1612.07565",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DCPT-16-63, NCTS-TH-1611",
    doi = "10.1103/PhysRevD.96.026017",
    journal = "Phys. Rev. D",
    volume = "96",
    number = "2",
    pages = "026017",
    year = "2017"
}
@article{Mikhaylov:2014aoa,
    author = "Mikhaylov, Victor and Witten, Edward",
    title = "{Branes And Supergroups}",
    eprint = "1410.1175",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/s00220-015-2449-y",
    journal = "Commun. Math. Phys.",
    volume = "340",
    number = "2",
    pages = "699--832",
    year = "2015"
}
@article{Jafarzade:2017fsc,
    author = "Jafarzade, Shahriyar and Nazari, Zainab",
    title = "{A New Integrable Ising-type Model from 2d $\mathcal{N}$=(2,2) Dualities}",
    eprint = "1709.00070",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "8",
    year = "2017"
}
@article{Deger:2018kur,
    author = "Deger, N.S. and Nazari, Z. and Sarioglu, O.",
    title = "{Supersymmetric solutions of N=(1,1) general massive supergravity}",
    eprint = "1803.06926",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.97.106022",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "10",
    pages = "106022",
    year = "2018"
}

@article{Bastian:2018fba,
    author = "Bastian, Brice and Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Five-Dimensional Gauge Theories from Shifted Web Diagrams}",
    eprint = "1810.05109",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.99.046012",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "4",
    pages = "046012",
    year = "2019"
}
@article{Sugimoto:2015nha,
    author = "Sugimoto, Yuji",
    title = "{The Enhancement of Supersymmetry in M-strings}",
    eprint = "1508.02125",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "OU-HET-867",
    doi = "10.1142/S0217751X16500883",
    journal = "Int. J. Mod. Phys. A",
    volume = "31",
    number = "16",
    pages = "1650088",
    year = "2016"
}
@article{Iqbal:2015dra,
    author = "Iqbal, Amer and Khan, Ahsan Z. and Qureshi, Babar A. and Shabbir, Khurram and Shehper, Muhammad A.",
    title = "{Topological field theory amplitudes for A$_{N\ensuremath{-}1}$ fibration}",
    eprint = "1507.02662",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP12(2015)017",
    journal = "JHEP",
    volume = "12",
    pages = "017",
    year = "2015"
}
@article{Iqbal:2009ki,
    author = "Iqbal, Amer and Kozcaz, Can and Sohail, Tanweer",
    title = "{Periodic Schur Process, Cylindric Partitions and N=2* Theory}",
    eprint = "0903.0961",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "3",
    year = "2009"
}
@article{Iqbal:2004ne,
    author = "Iqbal, Amer and Kashani-Poor, Amir-Kian",
    title = "{The Vertex on a strip}",
    eprint = "hep-th/0410174",
    archivePrefix = "arXiv",
    reportNumber = "SMS-0402, SLAC-PUB-10804, SU-ITP-04-39",
    doi = "10.4310/ATMP.2006.v10.n3.a2",
    journal = "Adv. Theor. Math. Phys.",
    volume = "10",
    number = "3",
    pages = "317--343",
    year = "2006"
}
@article{Taki:2008hb,
    author = "Taki, Masato",
    title = "{Flop Invariance of Refined Topological Vertex and Link Homologies}",
    eprint = "0805.0336",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "UT-08-14",
    month = "5",
    year = "2008"
}

@article{Iqbal:2007ii,
    author = "Iqbal, Amer and Kozcaz, Can and Vafa, Cumrun",
    title = "{The Refined topological vertex}",
    eprint = "hep-th/0701156",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2009/10/069",
    journal = "JHEP",
    volume = "10",
    pages = "069",
    year = "2009"
}
@article{Iqbal:2012mt,
    author = "Iqbal, Amer and Kozcaz, Can",
    title = "{Refined topological strings on local $ {\mathrm{\mathbb{P}}}^2 $}",
    eprint = "1210.3016",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-PH-TH-2012-244",
    doi = "10.1007/JHEP03(2017)069",
    journal = "JHEP",
    volume = "03",
    pages = "069",
    year = "2017"
}
@article{Neitzke:2004ni,
    author = "Neitzke, Andrew and Vafa, Cumrun",
    title = "{Topological strings and their physical applications}",
    eprint = "hep-th/0410178",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-04-A039",
    month = "10",
    year = "2004"
}

@article{Hollowood:2003cv,
    author = "Hollowood, Timothy J. and Iqbal, Amer and Vafa, Cumrun",
    title = "{Matrix models, geometric engineering and elliptic genera}",
    eprint = "hep-th/0310272",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-03-A074",
    doi = "10.1088/1126-6708/2008/03/069",
    journal = "JHEP",
    volume = "03",
    pages = "069",
    year = "2008"
}

@article{Hohenegger:2013ala,
    author = "Hohenegger, Stefan and Iqbal, Amer",
    title = "{M-strings, elliptic genera and $\mathcal{N} = 4$ string amplitudes}",
    eprint = "1310.1325",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-PH-TH-2013-237",
    doi = "10.1002/prop.201300035",
    journal = "Fortsch. Phys.",
    volume = "62",
    pages = "155--206",
    year = "2014"
}

@article{Duan:2018sqe,
    author = "Duan, Zhihao and Gu, Jie and Kashani-Poor, Amir-Kian",
    title = "{Computing the elliptic genus of higher rank E-strings from genus 0 GW invariants}",
    eprint = "1810.01280",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP03(2019)078",
    journal = "JHEP",
    volume = "03",
    pages = "078",
    year = "2019"
}
@article{Witten:1986bf,
    author = "Witten, Edward",
    title = "{Elliptic Genera and Quantum Field Theory}",
    reportNumber = "PUPT-1024",
    doi = "10.1007/BF01208956",
    journal = "Commun. Math. Phys.",
    volume = "109",
    pages = "525",
    year = "1987"
}

@article{Gomis:2008vc,
    author = "Gomis, Jaume and Rodriguez-Gomez, Diego and Van Raamsdonk, Mark and Verlinde, Herman",
    title = "{A Massive Study of M2-brane Proposals}",
    eprint = "0807.1074",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1126-6708/2008/09/113",
    journal = "JHEP",
    volume = "09",
    pages = "113",
    year = "2008"
}
@inproceedings{Gritsenko:1999nm,
    author = "Gritsenko, V.",
    title = "{Complex vector bundles and Jacobi forms}",
    eprint = "math/9906191",
    archivePrefix = "arXiv",
    month = "1",
    year = "1999"
}
@article{Haghighat:2013gba,
    author = "Haghighat, Babak and Iqbal, Amer and Koz\c{c}az, Can and Lockhart, Guglielmo and Vafa, Cumrun",
    title = "{M-Strings}",
    eprint = "1305.6322",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/s00220-014-2139-1",
    journal = "Commun. Math. Phys.",
    volume = "334",
    number = "2",
    pages = "779--842",
    year = "2015"
}
@article{Aharony:1997bh,
    author = "Aharony, Ofer and Hanany, Amihay and Kol, Barak",
    title = "{Webs of (p,q) five-branes, five-dimensional field theories and grid diagrams}",
    eprint = "hep-th/9710116",
    archivePrefix = "arXiv",
    reportNumber = "IASSNS-HEP-97-113, RU-97-81, SU-ITP-97-40",
    doi = "10.1088/1126-6708/1998/01/002",
    journal = "JHEP",
    volume = "01",
    pages = "002",
    year = "1998"
}
@article{Iqbal:2008ra,
    author = "Iqbal, Amer and Kozcaz, Can and Shabbir, Khurram",
    title = "{Refined Topological Vertex, Cylindric Partitions and the U(1) Adjoint Theory}",
    eprint = "0803.2260",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1016/j.nuclphysb.2010.06.010",
    journal = "Nucl. Phys. B",
    volume = "838",
    pages = "422--457",
    year = "2010"
}

@article{Haghighat:2011xx,
    author = "Haghighat, Babak and Vandoren, Stefan",
    title = "{Five-dimensional gauge theory and compactification on a torus}",
    eprint = "1107.2847",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP09(2011)060",
    journal = "JHEP",
    volume = "09",
    pages = "060",
    year = "2011"
}

@article{Haghighat:2012bm,
    author = "Haghighat, Babak and Manschot, Jan and Vandoren, Stefan",
    title = "{A 5d/2d/4d correspondence}",
    eprint = "1211.0513",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP03(2013)157",
    journal = "JHEP",
    volume = "03",
    pages = "157",
    year = "2013"
}


